Search for a light charged Higgs boson in the decay channel H+->csbar in ttbar events using pp collisions at sqrt(s) = 7 TeV with the ATLAS detector

A search for a charged Higgs boson (H+) in ttbar decays is presented, where one of the top quarks decays via t->H+b, followed by H+->two jets (csbar). The other top quark decays to Wb, where the W boson then decays into a lepton (e/mu) and a neutrino. The data were recorded in pp collisions at sqrt(s) = 7TeV by the ATLAS detector at the LHC in 2011, and correspond to an integrated luminosity of 4.7 fb-1. With no observation of a signal, 95% confidence level (CL) upper limits are set on the decay branching ratio of top quarks to charged Higgs bosons varying between 5% and 1% for H+ masses between 90 GeV and 150 GeV, assuming Br(H+->csbar)=100%.

==> abstract.tex <==
A search for a charged Higgs boson ($H^+$) in $\ttbar$ decays is presented, where one of the top 
quarks decays via $t\rightarrow H^+b$, followed by $H^+\rightarrow$ two jets ($\csbar$). The other
top quark decays to $Wb$, where the $W$~boson then decays into a lepton ($e/\mu$) and a neutrino.
The data were recorded in $pp$ collisions at $\sqrt{s} = 7$~TeV by the ATLAS detector 
at the LHC in 2011, and correspond to an integrated luminosity of 4.7 fb$^{-1}$.
With no observation of a signal, 
 95\% confidence level (CL) upper limits are set on the decay branching ratio 
 of top quarks to charged Higgs bosons varying between 5\% and 1\%
for $H^+$ masses between 90 GeV and 150 GeV, assuming ${\cal B}(H^+ \rightarrow c\bar{s})=100\%$.

{\bf PACS} 12.60.Fr,  14.65.Ha, 14.80.Da, 14.80.Fd

